Data Assimilation in the Latent Space of a Neural Network

There is an urgent need to build models to tackle Indoor Air Quality issue. Since the model should be accurate and fast, Reduced Order Modelling technique is used to reduce the dimensionality of the problem. The accuracy of the model, that represent a dynamic system, is improved integrating real data coming from sensors using Data Assimilation techniques. In this paper, we formulate a new methodology called Latent Assimilation that combines Data Assimilation and Machine Learning. We use a Convolutional neural network to reduce the dimensionality of the problem, a Long-Short-Term-Memory to build a surrogate model of the dynamic system and an Optimal Interpolated Kalman Filter to incorporate real data. Experimental results are provided for CO2 concentration within an indoor space. This methodology can be used for example to predict in real-time the load of virus, such as the SARS-COV-2, in the air by linking it to the concentration of CO2.

==> BackUp_Results.tex <==
\section{Results and Discussions}
In this section, we discuss how the structure of both AutoEncoder and LSTM is found, the results of the grid search for both datasets and the assimilation of the sensors data in both latent space and physical space. The data set is decomposed into training, validation and testing sets. The flow field and the associated CO\textsubscript{2} concentration does not change much between consecutive steps. For this reason, we decide to divide the data in training, validation and testing sets making jumps. First, the CFD output at timesteps corresponding to sensors data are excluded and are assigned to the testing set. For the remaining data, two consecutive timesteps are considered for the training, then a jump is performed. The jumped data, i.e the ones not considered yet, are assigned to the validation and testing sets alternately. Considering a jump equal to 1, this process is summarised in Figure~\ref{Fig:data_split}.

% \textcolor{red}{in total we have the sensors data for 10 timesteps}.

% Figure - Train, Validation and Test split
\begin{figure}
    \centering
    \includegraphics[width=1\textwidth]{img/train_test.pdf}
    \caption{Training, Validation and Testing sets. Two consecutive timesteps are considered for the training. The jumped data are assigned to the validation and testing sets alternately.}
    \label{Fig:data_split}
\end{figure}

%------------------%
%-- AutoEncoder -- %
%------------------%
\subsection{AutoEncoder}
The AutoEncoder implemented in this paper is a Convolutional AutoEncoder. Specifically, the Encoder is composed by some convolutional layers followed by a fully connected layer which determine the shape of the latent space. The decoder architecture is the mirror of the encoder one. The construction of the AutoEncoder is divided in two steps:
\begin{enumerate}
    \item The search of the structure;
    \item The Grid Search of hyper-parameters for each dataset.
\end{enumerate}

\subsubsection{Structure}
The search of the structure is conducted progressively. We start comparing few AutoEncoders (that, for example, differ on the number of hidden layers). We pick the best structure and we create new configurations to compare. We will call \textit{baseline} the model that we use to create new configurations. For each configuration we compute a 5-Cross Fold Validation and we choose the model with lower Mean-MSE and a low Std-MSE. A low standard deviation tells us that the model is stable and it does not depend on the data we use to train it and validate it. These experiments were run with Structured dataset. Once the structure was found, we considered the same structure also for RGB dataset. We fix the following parameters:
\begin{itemize}
    \item Number of filters: 32;
    \item Activation function: relu;
    \item Kernel size: 3x3;
    %\item Latent Space: 7
    \item Optimizer: adam;
    \item Number of epochs: 300;
    \item Batch size: 32.
\end{itemize}
The data we used for the CV are both train and validation sets. We shuffle the data before to start to make the neural network independent from the order of the data. We first check the good number of hidden Convolutional layers, listed \ref{List: lay_configurations}.


\begin{enumerate}
     \item Encoder with 3 Convolutional layers and Decoder with 4 Convolutional layers;
    \item Encoder with 4 Convolutional layers and Decoder with 5 Convolutional layers;
    \item Encoder with 5 Convolutional layers and Decoder with 6 Convolutional layers.
\end{enumerate}\captionof{enumcnt}[Autoencoder Convolutional layers configurations]{Autoencoder Convolutional layers configurations}\label{List: lay_configurations}

\vspace{0.5cm}
\noindent The configuration with the best performance is the number 2 with the results reported in Table \ref{tab:conf_2}. In Table \ref{tab:conf_2}, the column N indicates the number of the Autoencoder configuration.
\begin{table}[H]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}ccccccc@{}}
\toprule
\textbf{N} & \textbf{Mean-MSE} & \textbf{Std-MSE} & \textbf{Mean-MAE} & \textbf{Std-MAE} & \textbf{Mean-Time} & \textbf{Std-Time} \\ \midrule
1 & 1.324e-02 & 2.072e-02 & 5.573e-02 & 7.575e-02 & 775.665 & 5.606e+00 \\ \midrule
\textbf{2} & \textbf{2.435e-04} & \textbf{3.851e-05} & \textbf{1.034e-02} & \textbf{8.776e-04} & \textbf{812.293} & \textbf{1.436e+00} \\ \midrule
3 & 2.293e-02 & 2.763e-02 & 8.887e-02 & 9.818e-02 & 828.328 & 1.574e+00 \\ \bottomrule
\end{tabular}%
}
\caption[Autoencoder performance of the configurations with different convolutional layers]{Autoencoder performance of the configurations listed in List \ref{List: lay_configurations}. The column N indicates the number of the configuration. The bold row is the configuration with higher performance.}
\label{tab:conf_2}
\end{table}
\noindent Considering the model 2, we substitute the Convolutional layers with the Convolutional Transpose layers in the Decoder: configuration number 4. This configuration does not makes improvements to the first model, as we can see from Table \ref{tab:conv_transp}:
\begin{table}[H]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}ccccccc@{}}
\toprule
\textbf{N} & \textbf{Mean-MSE} & \textbf{Std-MSE} & \textbf{Mean-MAE} & \textbf{Std-MAE} & \textbf{Mean-Time} & \textbf{Std-Time} \\ \midrule
\textbf{2} & \textbf{2.435e-04} & \textbf{3.851e-05} & \textbf{1.034e-02} & \textbf{8.776e-04} & \textbf{812.293} & \textbf{1.436e+00} \\ \midrule
4 & 2.587e-04 & 4.114e-05 & 1.041e-02 & 9.384e-04 & 746.804 & 3.089e+00 \\ \bottomrule
\end{tabular}%
}
\caption[Autoencoder performance with Convolutional Transpose layers]{Autoencoder performance with Convolutional Transpose layers in the Decoder. The column N indicates the number of the configuration: the configuration 2 is the baseline and the configuration 4 is the one with the Convolutional Transpose layers.}
\label{tab:conv_transp}
\end{table}

\noindent Finally, we discard the Convolutional Transpose layers and we change the kernel size increasing it a little bit, shown in List \ref{List: ker_configurations}:

\begin{enumerate}
    \setcounter{enumi}{4}
    \item Kernel size equal to 5x5 everywhere;
    \item A mix of both sizes 3x3 and 5x5;
\end{enumerate}\captionof{enumcnt}[Autoencoder Kernel size configurations]{Autoencoder Kernel size configurations}\label{List: ker_configurations}

\vspace{0.5cm}
The configuration 5 is the best one but it is not better than the baseline, as we can see from Table \ref{tab:ker}.
\begin{table}[H]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}ccccccc@{}}
\toprule
\textbf{N} & \textbf{Mean-MSE} & \textbf{Std-MSE} & \textbf{Mean-MAE} & \textbf{Std-MAE} & \textbf{Mean-Time} & \textbf{Std-Time} \\ \midrule
\textbf{2} & \textbf{2.435e-04} & \textbf{3.851e-05} & \textbf{1.034e-02} & \textbf{8.776e-04} & \textbf{812.293} & \textbf{1.436e+00} \\ \midrule
5 & 1.055e-02 & 2.099e-02 & 4.460e-02 & 7.922e-02 & 1222.251 & 6.627e+00 \\ \midrule
6 & 1.058e-02 & 2.094e-02 & 4.650e-02 & 7.826e-02 & 1164.464 & 4.605e+00\\ \bottomrule
\end{tabular}%
}
\caption[Autoencoder performance with different kernel-sizes]{Autoencoder performance of the configurations listed in \ref{List: ker_configurations}. The column N indicates the number of the configuration: the configuration 2 is the baseline. }
\label{tab:ker}
\end{table}

\subsubsection{Grid Search}
For both datasets we make a grid search with the following parameters:
\begin{itemize}
    \item Number of filters: 16, 32, 64;
    \item Activation function: ReLu, Elu;
    \item Number of epochs: 250, 300, 400;
    \item Batch size: 16, 32, 64.
\end{itemize}
The Table \ref{tab:AE_hyper} shows the optimal hyper-parameters found for each dataset. Summarily, both datasets need the same hyper-parameters.
\begin{table}[H]
\centering
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{@{}ccccc@{}}
\toprule
\textbf{Dataset} & \textbf{Filters} & \textbf{Activation} & \textbf{Epochs} & \textbf{Batch size} \\ \midrule
\textbf{Structured} & 64 & ReLu & 400 & 32 \\ \midrule
\textbf{RGB} & 64 & ReLu & 400 & 16 \\ \bottomrule
\end{tabular}%
}
\caption[Autoencoder hyper-parameters for each dataset]{Autoencoder hyper-parameters for each dataset.}
\label{tab:AE_hyper}
\end{table}
\noindent The performance of both datasets are reported in Table \ref{Tab: AE_performance}. The results show that both datasets have very similar performance: low MSE and low standard deviation that means the model is not dependent on the set of input we choose to train it. The Mean-MSE is of the same order of magnitude: for the RGB dataset it is a little bit lower. The RGB dataset takes more time in training because an element of this dataset is composed of three channels, so it is the triple the Structured dataset.
\begin{table}[H]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccccc@{}}
\toprule
\textbf{DataSet} & \textbf{Mean-MSE} & \textbf{Std-MSE} & \textbf{Mean-MAE} & \textbf{Std-MAE} & \textbf{Mean-Time} & \textbf{Std-Time} \\ \midrule
Structured & 8.509e-05 & 1.577e-05 & 6.182e-03 & 8.714e-04 & 1887.612 & 6.845e+00 \\ \midrule
RGB & 3.670e-05 & 9.261e-06 & 3.601e-03 & 4.333e-04 & 2490.920 & 1.825e+01 \\ \bottomrule
\end{tabular}%
}
\caption[Autoencoder performance of both datasets with the best hyper-parameters]{Autoencoder performance of both datasets with the best hyper-parameters found with the Grid Search (Table \ref{tab:AE_hyper}}
\label{Tab: AE_performance}
\end{table}


\subsection{LSTM}
Here we did not use the CV but we computed the metrics repeating 5 times the fitting and the evaluation of the model. We use the original train set for fitting and the validation set for the validation. All data are encoded with the Autoencoder: each sample is a vector of 7 scalar. \\
We split the data in small sequences based on the number of timesteps we look back and the number of timesteps we want to predict. In this case, we predict one step forward and, assuming the number of steps we look back is equal to 3, the data are divided as Fig. \ref{Fig: lstm}.
\begin{figure}[H]
\centering
\includegraphics[width=0.7\textwidth]{img/lstm_data.pdf}
\caption[Data splitting for LSTM]{Data splitting for LSTM. The numerical subscript is the timestep: those in black are the timesteps we use to make the prediction and the red ones are the timestep we predict.}
\label{Fig: lstm}
\end{figure}

\subsubsection{Structure}
\noindent We followed the same strategy as for the Autoecoder: we before define the structure of the model and then we compute the grid search for each dataset.\\
We fix the following parameter:
\begin{itemize}
    \item Number of neurons: 30;
    \item Activation function: ReLu;
    \item Number of steps: 3;
    \item Optimizer: Adam;
    \item Number of epochs: 300;
    \item Batch size: 32.
\end{itemize}
For the structure, we try to stack from 1 to 5 LSTMs.
From an analysis of the results it can be seen that the model with the higher performance, as shown in Table \ref{tab:lstm_lay} is the single LSTM. 
\begin{table}[H]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}ccccccc@{}}
\toprule
\textbf{N} & \textbf{Mean-MSE} & \textbf{Std-MSE} & \textbf{Mean-MAE} & \textbf{Std-MAE} & \textbf{Mean-Time} & \textbf{Std-Time} \\ \midrule
\textbf{1} & \textbf{1.634e-02} & \textbf{2.510e-03} & \textbf{7.822e-02} & \textbf{8.553e-03} & \textbf{230.355} & \textbf{1.050e+00} \\ \midrule
2 & 2.822e-02 & 7.244e-03 & 1.060e-01 & 1.679e-02 & 360.877 & 6.618e-01 \\ \midrule
3 & 4.619e-02 & 1.942e-02 & 1.381e-01 & 3.034e-02 & 494.254 & 2.258e+00 \\ \midrule
4 & 5.020e-02 & 1.675e-02 & 1.414e-01 & 2.778e-02 & 658.039 & 2.632e+00 \\ \midrule
5 & 4.742e-02 & 1.183e-02 & 1.459e-01 & 2.075e-02 & 806.001 & 5.921e+00 \\ \bottomrule
\end{tabular}%
}
\caption[LSTMs performance]{LSTMs performance. The column N indicates the number of LSTMs we stacked. The bold row is the configuration with the best performance.}
\label{tab:lstm_lay}
\end{table}

\subsubsection{Grid Search}
\noindent Considering the LSTM model composed by one layer, we compute the grid search changing the hyper-parameters:
\begin{itemize}
    \item Number of neurons: 30, 50, 70;
    \item Activation function: ReLu, Elu;
    \item Number of steps: 3, 5, 7;
    \item Number of epochs: 200, 300, 400;
    \item Batch size: 16, 32, 64.
\end{itemize}
The Table \ref{Tab: LSTM_hyperparameters} shows the optimal hyper-parameters found for each dataset. The results show that RGB dataset needs more neurons and more observations back. 
\begin{table}[H]
\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{@{}ccclcc@{}}
\toprule
\textbf{Dataset} & \textbf{Neurons} & \textbf{Activation} & \textbf{Steps} & \textbf{Epochs} & \textbf{Batch size} \\ \midrule
\textbf{Structured} & 30 & Elu & 3 & 400 & 16 \\ \midrule
\textbf{RGB} & 50 & Elu & 7 & 400 & 16 \\ \bottomrule
\end{tabular}%
}
\caption[LSTM hyper-parameters for both datasets]{LSTM hyper-parameters for both datasets.}
\label{Tab: LSTM_hyperparameters}
\end{table}

\noindent From the Table \ref{Tab: LSTM_performance} we can see that RGB dataset performs better taking also less time.

\begin{table}[H]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccccc@{}}
\toprule
\textbf{DataSet} & \textbf{Mean-MSE} & \textbf{Std-MSE} & \textbf{Mean-MAE} & \textbf{Std-MAE} & \textbf{Mean-Time} & \textbf{Std-Time} \\ \midrule
Structured & 1.233e-02 & 1.398e-03 & 6.743e-02 & 3.428e-03 & 949.328 & 7.508e+00 \\ \midrule
RGB & 6.712e-03 & 6.704e-04 & 4.661e-02 & 3.004e-03 & 690.594 & 2.743e+00 \\ \bottomrule
\end{tabular}%
}
\caption[LSTM performance of both datasets with the best hyperarameters]{LSTM performance of both datasets with the best hyperarameters found with the Grid Search (Table \ref{Tab: LSTM_hyperparameters})}
\label{Tab: LSTM_performance}
\end{table}

\subsection{Data Assimilation in latent space}
In this phase, we used only the Test set. We encode it for both datasets using the corresponding Autoencoders. We did the same also for the Sensors data. \\
The assimilation will take place in the latent space. From the Test set, we select the sequences that predict the timesteps of sensors data. We make the prediction through the LSTM and we update the prediction using the corresponding observations through Optimal Interpolated Kalman Filter.
In the KF, the error covariance matrix $\hat{Q}$ is computed as $\hat{Q}=VV^T$ where $V$ is computed as described in \eqref{eq:covarianProcedure}. 
Since both predictions of the model and observations are values of CO\textsubscript{2} or pixels, i.e. the observations don't have to be transformed, the operator $\hat{H}$ is an identity matrix.\\
We studied how KF improves the accuracy of the prediction testing different values of $\hat{R}$ computed by the procedure in \eqref{eq:covarianProcedure} or, fixed as $\hat{R}=0.01\ I, 0.001\ I, 0.0001\ I$ where $I\in \mathbb{R}^{p\times p}$ denotes the identity matrix. This last assumption is usually made to give higher fidelity and trust to the observations.

The MSE of the background data in the latent space for the Structured dataset, without performing data assimilation is MSE$=7.220e-01$. Table \ref{Tab: LA_performanceLA} shows values of MSE after the assimilation in the latent space. It also reports values of execution time. As expected, we can observe an improvement in the execution time in assuming $\hat{R}$ as a diagonal matrix instead of a full matrix.

\begin{table}[H]
\centering
\begin{tabular}{@{}ccccccc@{}}
\toprule
${\bf \hat{R}}$ & \textbf{cov-matrix from data} & \textbf{0.01\ I} & \textbf{0.001\ I} & \textbf{0.0001 \ I}  \\ \midrule
${\bf MSE}$ & 3.215e-01 & 1.250e-02 & 1.787e-03 & 3.722e-05\\ \midrule
%\textbf{Condition Number} & 8.846e+03 & 6.322e+00 & 1.532e+00 & 1.053e+00 \\
\textbf{Time (sec)} & 2.053e-03 & 3.541e-04 & 2.761e-04 & 2.618e-04 \\ \bottomrule
\end{tabular}
\caption[MSE in the Latent space of the Latent Assimilation  for the Structured dataset]{Value of MSE of $h^a_t$ and execution time of the Latent Assimilation for different values of the observations errors covariance matrix $\hat{R}$ in the Latent space with the Structured dataset.}
\label{Tab: LA_performanceLA}
\end{table}

\noindent We have almost the same result for the RGB dataset. The MSE of the model without the assimilation is 5.447e-01. The assimilation increases the performance of the model but slower with respect to the Structured dataset. 

\begin{table}[H]
\centering
\begin{tabular}{@{}ccccccc@{}}
\toprule
${\bf \hat{R}}$ & \textbf{cov-matrix from data} & \textbf{0.01\ I} & \textbf{0.001\ I} & \textbf{0.0001 \ I}  \\ \midrule
${\bf MSE}$ & 2.444e-01 & 1.002e-02 & 4.409e-03 & 1.640e-03 \\ \midrule
%\textbf{Condition Number} & 8.846e+03 & 6.322e+00 & 1.532e+00 & 1.053e+00 \\
\textbf{Time (sec)} & 2.116e-03 & 5.245e-04 & 4.909e-04 & 4.830e-04 \\ \bottomrule
\end{tabular}
\caption[MSE in the Latent space of the Latent Assimilation for the RGB dataset]{Value of MSE of $h^a_t$ and execution time of the Latent Assimilation for different values of the observations errors covariance matrix $\hat{R}$ in the Latent space with the RGB dataset.}
\label{Tab: LA_performanceRGB}
\end{table}

%qui

\subsubsection{Physical space}
After performing DA in the latent space,  the results $h^a_t$ are reported in the physical space through the Decoder which gives $x^a_t$. Table \ref{Tab: LA_performance} and Table \ref{Tab: Post_DA} show values of MSE computed in the physical space after the assimilation performed with LA and with the standard methodology (standard DA) respectively. They also report values of execution time.  \\ 
The MSE in the physical space without the assimilation is MSE$=6.491e-02$ using the Structured dataset. Tables \ref{Tab: LA_performance} and \ref{Tab: Post_DA} show that both LA and DA improve the accuracy of the forecasting.  
Comparing the tables we can also observe that LA performs better both in terms of execution time and accuracy with respect to a Standard DA where the assimilation works directly with big matrices becoming very slow.

\begin{table}[H]
\centering
\begin{tabular}{@{}ccccccc@{}}
\toprule
${\bf \hat{R}}$ & \textbf{cov-matrix from data} & \textbf{0.01\ I} & \textbf{0.001\ I} & \textbf{0.0001\ I}  \\ \midrule
${\bf MSE}$ & 3.356e-02 & 6.933e-04 & 1.211e-04 & 2.691e-06 \\ \midrule
\textbf{Time (sec)} &  3.191e+00  & 2.899e+00  & 2.896e+00  & 2.896e+00 \\ 
\bottomrule
\end{tabular}
\caption[MSE in the Physical space of the Latent Assimilation with the Structured dataset]{Values of MSE of of $x^a_t$ in the Physical space for different values of the observations errors covariance matrix $\hat{R}$ with the Structured dataset.}
\label{Tab: LA_performance}
\end{table}
 
\begin{table}[H]
\centering
\begin{tabular}{@{}ccccccc@{}}
\toprule
${\bf R}$ & \textbf{cov-matrix from data} & \textbf{0.01\ I} & \textbf{0.001\ I} & \textbf{0.0001\ I} \\ \midrule
\textbf{MSE} & 5.179e-02 & 6.928e-03 & 6.928e-03 & 6.997e-03\\ \midrule
\textbf{Time (sec)} & 2.231e+03 & 2.148e+03 & 2.186e+03 & 2.159e+03\\ 
\bottomrule
\end{tabular}
\caption[MSE in the Physical space of the Standart Assimilation with the Structured dataset]{Standard Assimilation in the physical space performed by a  KF (see Equations~\eqref{Eq: StartKalman}-\eqref{eq:kalmananalysis}). Here $R \in \mathbb{R}^{n\times n}$ is defined in the physical space.}
\label{Tab: Post_DA}
\end{table}

\noindent Figures \ref{Fig: assimilation_509}, \ref{Fig: assimilation_1062} and \ref{Fig: assimilation_1485} show graphically the assimilation results of the timesteps 509, 1062 and 1485 respectively using the LA model. 

\begin{figure}[H]
\centering
    \subfigure[][Predicted state]{\includegraphics[width=0.45\textwidth]{img/LSTMpred_0.png}}
\hspace{2mm}
    \subfigure[][Observation]{\includegraphics[width=0.45\textwidth]{img/sensor_0.png}}
\hspace{2mm}
    \subfigure[][Updated state]{\includegraphics[width=0.45\textwidth]{img/3_0.png}}
\caption[Assimlation result with the Structured dataset at the timestep 509]{Assimlation result colored by Tracer field at the timestep 509 where (a) is the LSTM predicted state, (b) is the interpolated observation and (c) is the updated state obtained through the Optimal Kalman Filter}
\label{Fig: assimilation_509}
\end{figure}

\begin{figure}[H]
\centering
    \subfigure[][Predicted state]{\includegraphics[width=0.45\textwidth]{img/LSTMpred_2.png}}
\hspace{2mm}
    \subfigure[][Observation]{\includegraphics[width=0.45\textwidth]{img/sensor_2.png}}
\hspace{2mm}
    \subfigure[][Updated state]{\includegraphics[width=0.45\textwidth]{img/3_2.png}}
\caption[Assimlation result at the timestep 1062]{Assimlation result with the Structured dataset colored by Tracer field at the timestep 1062 where (a) is the LSTM predicted state, (b) is the interpolated observation and (c) is the updated state obtained through the Optimal Kalman Filter}
\label{Fig: assimilation_1062}
\end{figure}

\begin{figure}[H]
\centering
    \subfigure[][Predicted state]{\includegraphics[width=0.45\textwidth]{img/LSTMpred_4.png}}
\hspace{2mm}
    \subfigure[][Observation]{\includegraphics[width=0.45\textwidth]{img/sensor_4.png}}
\hspace{2mm}
    \subfigure[][Updated state]{\includegraphics[width=0.45\textwidth]{img/3_4.png}}
\caption[Assimlation result with the Structured dataset at the timestep 1485]{Assimlation result colored by Tracer field at the timestep 1485 where (a) is the LSTM predicted state, (b) is the interpolated observation and (c) is the updated state obtained through the Optimal Kalman Filter}
\label{Fig: assimilation_1485}
\end{figure}


\subsubsection{Increasing the latent space}
We tried to increase the size of the latent space. For computational reasons, we run the experiments with the Structured dataset only.
The Table \ref{Tab: LS_latent} and \ref{Tab: LS_physical} contain the MSE values of the Latent Assimilation model with different latent space sizes, from 1000 to 20000, computed in the latent  and physical space respectively. The column "No DA" reports the MSE values without the assimilation. We observe that defining $\hat{R}$ as an identity matrix there are improvements.

\begin{table}[H]
\centering
\begin{tabular}{@{}ccccccc@{}}
\toprule
\textbf{Latent Space} & \textbf{No DA} & \textbf{0.01\ I} & \textbf{0.001\ I} & \textbf{0.0001 \ I}  \\ \midrule
1000 & 4363e-03 & 5.141e-04 & 4.980e-04 & 4.961e-04\\ \midrule
3000 & 6.472e-04 & 9.933e-05 & 9.566e-05 & 9.501e-05\\ \midrule
5000 & 6.012e-04 & 1.009e-04 & 9.184e-05 & 9.076e-05\\ \midrule
7000 & 7.295e-04 & 1.179e-04 & 1.146e-04 & 1.142e-04\\ \midrule
12000 & 1.727e-04 & 3.651e-05 & 3.540e-05 & 3.531e-05\\ \midrule
15000 & 1.660e-04 & 3.529e-05 & 3.463e-05 & 3.457e-05\\ \midrule
18000 & 2.941e-04 & 3.141e-05 & 3.086e-05 & 3.085e-05\\ \midrule
20000 & 3.465e-04 & 6.506e-05 & 6.177e-05 & 6.073e-05\\ \bottomrule
\end{tabular}
\caption[MSE values in the latent space of LA with different latent space sizes]{MSE values of LA model in the latent space with different latent space sizes. The column Latent Space indicates the size of the latent space, the column No DA indicates the MSE of the model without the assimilation and the other columns indicate the MSE of the LA model with different observation error covariance matrix $\hat{R}$}
\label{Tab: LS_latent}
\end{table}

\begin{table}[H]
\centering
\begin{tabular}{@{}ccccccc@{}}
\toprule
\textbf{Latent Space} & \textbf{No DA} & \textbf{0.01\ I} & \textbf{0.001\ I} & \textbf{0.0001 \ I}  \\ \midrule
1000 & 3.532e-02  & 1.347e-03 & 1.278e-03 & 1.278e-03\\ \midrule
3000 & 3.261e-02  & 1.828e-03 & 1.694e-03 & 1.653e-03\\ \midrule
5000 & 2.822e-02  & 1.975e-03 & 1.689e-03 & 1.667e-03\\ \midrule
7000 & 3.352e-02  & 1.248e-03 & 1.171e-03 & 1.155e-03\\ \midrule
%10000 & 1.727e-04 & 3.651e-05 & 3.540e-05 & 3.531e-05\\ \midrule
12000 & 2.479e-02 & 1.248e-03 & 1.171e-03 & 1.155e-03\\ \midrule
15000 & 1.734e-02 & 1.325e-03 & 1.262e-03 & 1.253e-03\\ \midrule
18000 & 2.941e-04 & 1.080e-03 & 9.848e-04 & 9.743e-04\\ \midrule
20000 & 2.514e-02 & 1.621e-03 & 1.424e-03 & 1.365e-03\\ \bottomrule
\end{tabular}
\caption[MSE values in the physical space of LA with different latent space sizes]{MSE values of LA model in the physical space with different latent space sizes. The column Latent Space indicates the size of the latent space, the column No DA indicates the MSE of the model without the assimilation and the other columns indicate the MSE of the LA model with different observation error covariance matrix $\hat{R}$}
\label{Tab: LS_physical}
\end{table}

Table \ref{Tab: LS_latent_time} and \ref{Tab: LS_physical_time} show the time values for each latent space sizes in the latent and physical space respectively

\begin{table}[H]
\centering
\begin{tabular}{@{}cccccc@{}}
\toprule
\textbf{Latent Space} & \textbf{0.01\ I} & \textbf{0.001\ I} & \textbf{0.0001 \ I}  \\ \midrule
1000 & 5.637e-01 & 5.525e-01 & 5.637e-01 \\ \midrule
3000 & 2.272e+00 & 2.260e+00 & 2.147e+00\\ \midrule
5000 & 5.197e+00 & 5.301e+00 & 5.358e+00\\ \midrule
7000 & 1.104e+01 & 1.125e+01 & 1.136e+01\\ \midrule
12000 & 4.289e+01 & 4.353e+01 & 4.375e+01\\ \midrule
15000 & 7.960e+01 & 8.072e+01 & 8.180e+01\\ \midrule
18000 & 1.432e+02 & 1.441e+02 & 1.443e+02\\ \midrule
20000 & 2.096e+02 & 2.124e+02 & 1.997e+02\\ \bottomrule
\end{tabular}
\caption[Time values in the latent space of LA with different latent space sizes]{Time values of LA model in the latent space with different latent space sizes. The column Latent Space indicates the size of the latent space, the other columns indicate the time of the LA model with different observation error covariance matrix $\hat{R}$}
\label{Tab: LS_latent_time}
\end{table}

\begin{table}[H]
\centering
\begin{tabular}{@{}cccccc@{}}
\toprule
\textbf{Latent Space} & \textbf{0.01\ I} & \textbf{0.001\ I} & \textbf{0.0001 \ I}  \\ \midrule
1000 & 5.478e-01 & 5.561e-01 & 5.461e-01 \\ \midrule
3000 & 2.137e+00 & 2.115e+00 & 2.134e+00\\ \midrule
5000 & 5.300e+00 & 5.413e+00 & 5.535e+00\\ \midrule
7000 & 1.110e+01 & 1.113e+01 & 1.144e+01\\ \midrule
12000 & 4.390e+01 & 4.324e+01 & 4.421e+01\\ \midrule
15000 & 7.953e+01 & 8.171e+01 & 8.071e+01\\ \midrule
18000 & 1.497e+02 & 1.476e+02 & 1.454e+02\\ \midrule
20000 & 1.937e+02 & 2.052e+02 & 2.009e+02\\ \bottomrule
\end{tabular}
\caption[Time values in the physical space of LA with different latent space sizes]{Time values of LA model in the physical space with different latent space sizes. The column Latent Space indicates the size of the latent space, the other columns indicate the time of the LA model with different observation error covariance matrix $\hat{R}$}
\label{Tab: LS_physical_time}
\end{table}

==> BackUp_SetupRealCase.tex <==
\section{Set up of a real test case}

: they constitute a time series composed by 3500 time-steps . Each time-step is described with a PVTU file that stands for ParaView Parallel (Partitioned) VTK Unstructured Data (Kitware Inc.).
ParaView is an application designed based on the Visualization Toolkit (VTK) library \cite{book}. We use it to visualize and manipulate the data.
ParaView is an application designed with the need to visualize large data sets in mind. It is based on the Visualization Toolkit (VTK) library. The VTK library is an open source software for manipulating and displaying scientific data \cite{VTK}. We used directly VTK library to manage the data. \\
Each PVTU file contains the information about all the domain represented as a mesh, Figure \ref{Fig: ClarenceCentre_mesh}.

In Figure \ref{Fig:mesh} is shown the mesh colored by Tracer Field where the blue color means low C02 concentration and red color indicates high value of concentration. The Figure \ref{Fig: mesh_a} is the all domain, while the Figure \ref{Fig: mesh_b} is the room chosen for the test case.
\begin{figure}[H]
\centering
    \subfigure[]{\includegraphics[width=0.45\textwidth]{img/mesh.pdf}\label{Fig: mesh_a}}
\hspace{2mm}
    \subfigure[]{\includegraphics[width=0.45\textwidth]{img/indoor.pdf}\label{Fig: mesh_b}}
\caption[The unstructured mesh of the domain colored by Tracer field]{The unstructured mesh of the all domain (a) and the zoomed room mesh (b) colored by Tracer field.}
\label{Fig:mesh}
\end{figure}

\begin{itemize}
    \item Data from the unstructured 2D slice are projected on a structured grid, named later ``Structured dataset". %Create new points for the slice. We call these data "Structured dataset"
    \item Data from the unstructured 2D slice are directly converted into RGB screenshot based on the CO\textsubscript{2} values, named later ``RGB dataset". % of the room and cut a slice represented by a RGB screenshot colored based on CO\textsubscript{2} values. We call these data "RGB dataset"
\end{itemize}

\subsubsection{Structured Dataset}
We build new points from the original mesh but this time in a structured way. Considering the x, y, z coordinates of the room in the domain and the height, width, depth of the room we create new points: we can image these points like a matrix with shape 180x250 located halfway up the room (see Figure \ref{Fig:StructuredDS}). For this purpose, we first create the coordinates for each point and then we use the Probe Filter.
The Probe Filter \cite{book} takes as input the Source and the new positions where we want to compute the attributes through the interpolation. In this case, the Source is the original mesh.
ProbeFilter is a filter that computes point attributes (e.g., scalars, vectors, etc.) at specified point positions. The filter has two inputs: the Input and the Source. The Input geometric structure is passed through the filter. The point attributes are computed at the Input point positions by interpolating into the source data \cite{Probe}. In this case, the Source is the original mesh.\\
This process is done for each time step.

\subsubsection{RGB Dataset}
The ``RGB dataset" is directly generated from the 2D slice to create the corresponding RGB image: a screenshot of the slice coloured based on the CO\textsubscript{2} concentration values is created. The scalar bar of the RGB images is set based on the minimum and maximum CO\textsubscript{2} concentration, i.e. 400 ppm and 1420 ppm, respectively. This transformation allows to move from unstructured mesh to structured data since the RGB image is a 3D matrix of pixel values. The final size of the RGB images is 180$\times$250 and are shown in Figure~\ref{Fig:rgb_cut}.


% We looked for the global minimum and maximum of CO\textsubscript{2} values present in both Structured dataset and sensors data: they are respectively 400 ppm and 1420 ppm.  We set the scalar bar of the RGB images to this range. With the screenshot, we move from unstructured mesh to structured data since the RGB image is a 3D matrix of pixel values. The size of the RGB images is 215$\times$260 and it includes the background (Figure \ref{Fig:rgb}).
% The second dataset we want to create is composed by images (screenshots). To extract the room we used the node ids of the room: using only the node ids we don't have a mesh, but only the isolated points. Indeed, we re-built the unstructured mesh of the room using the Delaunay3D filter.
% The Delaunay3D filter \cite{book} builds a new unstructured mesh starting from a list of input points. We applied the Delaunay filter for each time-step.
% The last step was to extract the slice and create the corresponding RGB image. 
% Here we used a different library: Pyvista \cite{sullivan2019pyvista}.
% To slice the room, we set the x, y and z coordinates in such a way that the slice is always at the half of the height of the room. 
% We make a screenshot of the slice coloured based on Tracer values. 
%Delaunay3D is a filter that constructs a 3D Delaunay triangulation from a list of input points. These points may be represented by any dataset of type PointSet and subclasses. The output of the filter is an unstructured grid dataset \cite{Delaunay3D}. We applied the Delaunay filter for each time-step.
%PyVista (formerly vtki) is a helper module for the Visualization Toolkit (VTK) that takes a different approach on interfacing with VTK through NumPy and direct array access. This package provides a Pythonic, well-documented interface exposing VTK’s powerful visualization back-end to facilitate rapid prototyping, analysis, and visual integration of spatially referenced dataset \cite{Pyvista}.

% \begin{figure}
% \centering
%     \subfigure[]{\includegraphics[width=0.45\textwidth]{img/300.png}}
% \hspace{2mm}
%     \subfigure[]{\includegraphics[width=0.45\textwidth]{img/600.png}}
% \hspace{2mm}
%     \subfigure[]{\includegraphics[width=0.45\textwidth]{img/900.png}}
% \hspace{2mm}
%     \subfigure[]{\includegraphics[width=0.45\textwidth]{img/1200.png}}
% \hspace{2mm}
%     \subfigure[]{\includegraphics[width=0.45\textwidth]{img/1500.png}}
% \hspace{2mm}
%     \subfigure[]{\includegraphics[width=0.45\textwidth]{img/1800.png}}
% \caption[The RGB screenshots colored by Tracer field]{The RGB screenshots colored by Tracer field at time-steps (a) 300, (b) 600, (c) 900, (d) 1200, (e) 1500 and (f) 1800.}
% \label{Fig:rgb}
% \end{figure}

We can note that the colored pixels are not aligned cause of the irregular nature of the mesh.
These data are bigger than Structured data. For this reason, we extract a centered sub-image of shape 180x250 from RGB data. This sub-image contains a very small part of the background and we fill these background pixels with the values of the pixel in the next row (or column if we are moving on x-axis). The result is shown in Figure \ref{Fig:rgb_cut}.

\begin{figure}[H]
\centering
    \subfigure[]{\includegraphics[width=0.45\textwidth]{img/300_cut.png}}
    \label{Fig: 300_cut}
\hspace{2mm}
    \subfigure[]{\includegraphics[width=0.45\textwidth]{img/600_cut.png}}
    \label{Fig: 600_cut}
\hspace{2mm}
    \subfigure[]{\includegraphics[width=0.45\textwidth]{img/900_cut.png}}
    \label{Fig: 900_cut}
\hspace{2mm}
    \subfigure[]{\includegraphics[width=0.45\textwidth]{img/1200_cut.png}}
    \label{Fig: 1200_cut}
\hspace{2mm}
    \subfigure[]{\includegraphics[width=0.45\textwidth]{img/1500_cut.png}}
    \label{Fig: 1500_cut}
\hspace{2mm}
    \subfigure[]{\includegraphics[width=0.45\textwidth]{img/1800_cut.png}}
    \label{Fig: 1800_cut}
\caption[The processed RGB screenshots colored by Tracer field]{The processed RGB screenshots colored by Tracer field at time-steps (a) 300, (b) 600, (c) 900, (d) 1200, (e) 1500 and (f) 1800.}
\label{Fig:rgb_cut}
\end{figure}

\subsection{Sensors Data Pre-Process}
In \cite{song2018natural} the research team designed its own monitor units with seven sensors, which enabled simultaneous measurements of carbon
dioxide (CO2), carbon monoxide (CO), nitrogen dioxide (NO2), temperature, relative humidity (RH) and barometric pressure to be made. In the room the sensors are located in different positions and heights (Fig. \ref{Fig: sensors}).
\begin{figure}[H]
\centering
\includegraphics[width=0.5\textwidth]{img/sensors_pos.PNG}
\caption[Sensors positions in the room]{Sensors positions in the room.}
\label{Fig: sensors}
\end{figure}

\noindent We computed the sensors position in our matrix of the shape 180x250.
Considering the size of the room and the shape of the matrix, we computed the number of pixel corresponding to one pixel in both axis: about 3 pixels per cm in both axis.
We choose to expand the value of each sensor in a radius of 30cm: in the matrix, this corresponds to a radius of 10 pixels (Figure  \ref{Fig: sensor_pos}).

\begin{figure}[H]
\centering
    \subfigure[]{\includegraphics[width=0.45\textwidth]{img/sensorpos_0.png}}
\hspace{2mm}
    \subfigure[]{\includegraphics[width=0.45\textwidth]{img/sensorpos_1.png}}
\hspace{2mm}
    \subfigure[]{\includegraphics[width=0.45\textwidth]{img/sensorpos_2.png}}
\hspace{2mm}
    \subfigure[]{\includegraphics[width=0.45\textwidth]{img/sensorpos_3.png}}
\hspace{2mm}
    \subfigure[]{\includegraphics[width=0.45\textwidth]{img/sensorpos_4.png}}
\hspace{2mm}
    \subfigure[]{\includegraphics[width=0.45\textwidth]{img/sensorpos_5.png}}
\caption[Expansion of the sensors values]{The results of the expansion of the sensor values in a radius of 30cm colored by Tracer field at time-steps 509 (a), 643 (b), 1062 (c), 1359 (d), 1485 (e), 1741 (f).}
\label{Fig: sensor_pos}
\end{figure}

\noindent The value of the sensors are stored in a file excel: in total, we have the data of each sensor for 10 time-steps.
Once we expanded the values of sensors in the radius, we linearly interpolated the values using the Scipy library (Figure \ref{Fig: sensor_prep}). The interpolation is repeated for each time-step. The result of this process is good for the Structured dataset. We also create the RGB version of these data to make the assimilation with the RGB dataset.

\begin{figure}[H]
\centering
    \subfigure[]{\includegraphics[width=0.45\textwidth]{img/sensor_0.png}}
\hspace{2mm}
    \subfigure[]{\includegraphics[width=0.45\textwidth]{img/sensor_1.png}}
\hspace{2mm}
    \subfigure[]{\includegraphics[width=0.45\textwidth]{img/sensor_2.png}}
\hspace{2mm}
    \subfigure[]{\includegraphics[width=0.45\textwidth]{img/sensor_3.png}}
\hspace{2mm}
    \subfigure[]{\includegraphics[width=0.45\textwidth]{img/sensor_4.png}}
\hspace{2mm}
    \subfigure[]{\includegraphics[width=0.45\textwidth]{img/sensor_5.png}}
\caption[Interpolation of the observations colored by Tracer field ]{The results of the linear interpolation of the observations colored by Tracer field at time-steps 509 (a), 643 (b), 1062 (c), 1359 (d), 1485 (e), 1741 (f).}
\label{Fig: sensor_prep}
\end{figure}
